ADG-Pose: Automated Dataset Generation for Real-World Human Pose Estimation

Recent advancements in computer vision have seen a rise in the prominence of applications using neural networks to understand human poses. However, while accuracy has been steadily increasing on State-of-the-Art datasets, these datasets often do not address the challenges seen in real-world applications. These challenges are dealing with people distant from the camera, people in crowds, and heavily occluded people. As a result, many real-world applications have trained on data that does not reflect the data present in deployment, leading to significant underperformance. This article presents ADG-Pose, a method for automatically generating datasets for real-world human pose estimation. These datasets can be customized to determine person distances, crowdedness, and occlusion distributions. Models trained with our method are able to perform in the presence of these challenges where those trained on other datasets fail. Using ADG-Pose, end-to-end accuracy for real-world skeleton-based action recognition sees a 20% increase on scenes with moderate distance and occlusion levels, and a 4X increase on distant scenes where other models failed to perform better than random.

==> equations/f1.tex <==
\begin{equation} \label{eq:f1}
    F1 = 2*\frac{Precision * Recall}{Precision + Recall}
\end{equation}

==> equations/map.tex <==
\begin{multicols}{2}
    \begin{equation} \label{eq:mAP}
        Precision = \frac{TP}{TP+FP}
    \end{equation}\break 
    \begin{equation} \label{eq:mRC}
        Recall = \frac{TP}{TP+FN}
    \end{equation}
\end{multicols}

==> tab/action.tex <==
\begin{table}[t]
    \centering
    \small
    \resizebox{\linewidth}{!}{
        \begin{tabular}{C{1.15cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}|C{0.95cm}}
            Camera & Walk & Throw & Dig & Trunk & Clap & Box & Wave & Run & Jog & Carry & Total \\
            \hline
            \hline
            \multicolumn{12}{c}{trained on COCO} \\
            \hline
            Ground  &55.6	&55.6	&55.6  &100.0	&55.6	&33.3	&77.8	&55.6	&55.6	&55.6 &60.0 \\
            Roof   &  0.0&  0.0&  0.0&  0.0&  100.0&  0.0&  0.0&  0.0&  0.0&  0.0& 10.0 \\
            \hline
            \multicolumn{12}{c}{trained on generated dataset} \\
            \hline
            Ground  &77.8 &100.0	&77.8  &100.0	&88.9 &55.6		&77.8	&77.8	&88.9	&66.7  &81.1 \\
            Roof   & 66.6 & 22.2 & 00.0 & 44.4 & 11.1 & 77.7 & 22.2 & 33.3 & 44.4 & 77.7 & 40.0 \\
        \end{tabular}
    }
    \caption{Accuracy of end-to-end action recognition on UCF-ARG. Results obtained by feeding EfficientHRNet-H$_0$ keypoint predictions into a skeleton-based ST-GCN. \vspace{-10pt}}
    \label{tab:action}
\end{table}

==> tab/dataset_distributions.tex <==
\capbtabbox{
    %\vspace{-12pt}
    \centering
    %\resizebox{0.4\linewidth}{!}{
        \begin{tabular}{c|c|c|c|c|c}
                                & Persons   & Average & \multicolumn{3}{c}{\% Resolution} \\
            Dataset             & per Image & IoU     & $Q_1$   & $Q_2$   & $Q_3$     \\
            \hline \hline                                                                              
            MPII                & 1.6       & 0.11    & -     & -     & -       \\
            AI Challanger       & 2.33      & 0.12    & -     & -     & -       \\
            COCO                & 1.25      & 0.11    & 0.484 & 0.693 & 0.853   \\
            CrowdPose           & 4         & 0.27    & 0.425 & 0.644 & 0.814   \\
            OCHuman             & 1.72      & 0.67    &       &       &         \\
            Tiny People Pose    & 2.93      & -       & -     & -     & -       \\
            \hline
            \textbf{Ours}                & \textbf{9.33}      & \textbf{0.33}    & \textbf{0.105} & \textbf{0.183} & \textbf{0.316}   \\
            
        
            
            %\hline
        \end{tabular}%
        %\caption{Distribution comparisons with State-of-the-Art datasets.}%    
        \label{tab:cocotest-dev}
}%\vspace{-20pt}



==> tex/Setup.tex <==
\section{Experimental Setup} \label{sec:Setup}

To validate the efficacy of our proposed method, we train a bottom-up pose estimator our newly constructed dataset for comparisons with a COCO \cite{COCO} trained version. For the model we choose EfficientHRNet \cite{EfficientHRNet}. Its lightweight nature and real-time capabilities are befitting of real-world applications and its scalability will allow us to test with different configurations. We look at the H$_0$ model and using the methodology present in \cite{EfficientHRNet} we scale up to create an H$_1$ version as well, using EfficientNet-B1 \cite{efficientnet} as a backbone. Keeping with the scaling, we utilize input resolutions of 512 and 544 for the COCO trained model, but increase the latter to 768 for the model trained on our dataset. As COCO images are lower resolution than those in our dataset, further increasing resolution for COCO training does not noticeably increase accuracy, as demonstrated in \cite{higherhrnet}. EfficientHRNet by default limits the number of detections to 30, fitting with the COCO dataset. To more fairly compare, we take the same approach when training and validating with our dataset. Training starts with a pretrained weights and is fine-tuned for 150 epochs with a learning rate of $1e-5$ for the H$_0$ model and $1e-6$ for the larger H$_1$ model. To increase training speed, images are scaled to the input resolution offline.
